Schedulability Analysis of WSAN Applications: Outperformance of A Model Checking Approach

Wireless sensor and actuator networks (WSAN) are real-time systems which demand high degrees of reliability requirements. To ensure this level of reliability, different analysis approaches have been proposed for WSAN applications. Among different alternatives, analytical analysis and model checking are two common approaches which are widely used for the formal analysis of WSAN applications. Analytical approaches apply constraint satisfaction methods, whereas model checking generates explicit states of models and analyze them. In this paper, we compare the two approaches in schedulability analysis of WSAN applications using an application for monitoring and control of civil infrastructures, which is implemented on the Imote2 wireless sensor platform. We show how the highest possible data acquisition frequency for this application is computed while meeting the deadlines, and compare the results of the two approaches as well as their scalability, extensibility, and flexibility.

==> 06-Related.tex <==
\section{Related work}\label{sec::related}

A major requirement for real-time systems is to provide an accurate prediction of timing. In order to guarantee that the actions in real-time systems meet their respective deadlines, schedulability analysis have been developed~\cite{sha2004real}. Several techniques have been proposed to provide such predictions, including utilization-based tests~\cite{Liu_JACM73}, response time analysis~\cite{Joseph_CJ86}, real-time calculus~\cite{Thiele_IEEE00} and model checking approaches~\cite{Waszniowski2008}~\cite{Yi_tool04}. Although each of the above mentioned techniques have a strong motivation to be used in real-time schedulability analysis, very few works compared them against each other. 
The main reason is that the techniques are normally optimized for specific applications, which makes it difficult to globally compare the techniques. 
There are very few works addressing the advantages and drawbacks of the analytical analysis approaches (i.e., response time analysis, utilization-based, real-time calculus) and the model checking approaches compared to each other, which is the main target of this paper. 

Among the works that analyzed a real-time system using model checking approaches is a formal semantics and a language, Real-Time Specification Language (RTSL), which is developed in~\cite{Fredette_RTSS93}. The reachability analysis and the formal semantics help to explore the entire state space and check whether any deadline has missed in a state. Similarly, other works used various approaches, such as Petri Nets to check the behavior of task executions~\cite{Furfaro_MCSIT07}~\cite{Xu_IEEE02}. 

In the context of uniprocessor real-time systems, the authors in~\cite{Fersman_tools02} developed a timed automata model for schedulability analysis of preemptable tasks that have interaction with each other through synchronization methods. Moreover, a technique in~\cite{Li_IPDPSW10} is proposed to tackle similar problem in analyzing tasks executing synchronously. The work in~\cite{Fersman_JC04} extended the reachability analysis on timed automata to consider precedence and resource constraints in uniprocessor real-time systems. Similar techniques have been used in multiprocessor real-time systems domain, with the goal of providing an exact analysis for the systems. The authors in~\cite{Sheng_WMTV10} proposed a schedulability analysis based on model checking for multiprocessor real-time systems. The main motivation for using the model checking approach in the paper is the need for an exact approach in multi-core systems by exploring the entire state space and check the properties. The comparison with analytical analysis shows less pessimism in the model checking approach with the cost of handling less number of cores in the model. Similarly, the authors in~\cite{Guan_ISORC08} proposed a model checking approach for an exact schedulability analysis of multi-core real-time systems, leading to the same conclusion as in~\cite{Sheng_WMTV10}. 

Study of the state of the art shows that adopting analysis techniques is highly dependent on the model and application. This paper compares an analytical approach based on response time and a model checking approach on a WSAN application to provide an evidence on the benefits and drawbacks of each. 




















